Dynamical Surface Imaging of lambda Andromedae

We present temperature maps of RS CVn star lambda Andromedae, reconstructed from interferometric data acquired in 2010 and 2011 by the MIRC instrument at the Center for High Angular Resolution Astronomy Array. To constrain the stellar parameters required for this imaging task, we first modeled the star using our GPU-accelerated code SIMTOI. The stellar surface was then imaged using our open source interferometric imaging code ROTIR, in the process further refining the estimation of stellar parameters. We report that the measured angular diameter is 2.742 +/- 0.010 mas with a limb-darkening coefficient of 0.231 +/- 0.024. While our images are consistent with those of prior works, we provide updated physical parameters for lambda Andromedae (R_star = 7.78 +/- 0.05 R_odot, M_star = 1.24 +/- 0.72 M_odot, log L/L_odot = 1.46 +/- 0.04).

==> Martinez_etal_2021 - Dynamical Surface Imaging of lambda Andromedae/tables/calibrators.tex <==
\begin{deluxetable*}{lCcc}[t!]
\tablenum{2}
\tablecaption{Calibrators for $\lambda$ Andromedae \label{tab:cals}}
\tablecolumns{4}
\tablewidth{0pt}
\tablehead{
\colhead{Calibrator Name} &
\colhead{Calibrator Size} &
\colhead{Source} &
\colhead{Epoch Used} \vspace{-5pt} \\
\colhead{} &
\colhead{(mas)} &
\colhead{} &
\colhead{}
}
\startdata
7 And (HD 219080) & 0.65 \pm 0.03 & \cite{mourard:2015} & 2010 \\
37 And (HD 5448) & 46.66 \pm 0.06 & \cite{roettenbacher:2016a}\tablenotemark{a} & 2010 \\
$\sigma$ Cyg (HD 202850) & 0.542 \pm 0.021 & \cite{zhao:2008} & 2010 \\
\hline
7 And (HD 219080) & 0.676 \pm 0.047 & SearchCal \citep{bonneau:2006} & 2011 \\
$\sigma$ Cyg (HD 202850) & 0.54 \pm 0.02 & \cite{barnes:1978} & 2011 \\
22 And (HD 571) & 0.591 \pm 0.041 & SearchCal \citep{bonneau:2006} & 2011 \\
HR 653 (HD 13818) & 0.646 \pm 0.045 & SearchCal \citep{bonneau:2006} & 2011 \\
$\eta$ Aur (HD 32630) & 0.336 \pm 0.023 & SearchCal \citep{bonneau:2006} & 2011 \\
\enddata
\tablecomments{The angular sizes for the 2011 epochs are based on what was reported from \cite{parks:2021} since we use their reduced and calibrated data. We use updated angular sizes for each calibrator star in the 2010 epoch since we do a new and separate reduction and calibration. The differences in angular sizes for 7~And and $\sigma$ Cyg used between the two years are small and within their 1$\sigma$ errors.
\tablenotetext{a}{This is the semi-major axis angular separation of the binary calculated by \cite{roettenbacher:2016a}.}}
\end{deluxetable*}


==> Martinez_etal_2021 - Dynamical Surface Imaging of lambda Andromedae/tables/lambdaAndparams.tex <==
\begin{deluxetable*}{lCcCl}%[t!]
\tablenum{4}
\tablecaption{Final $\lambda$ Andromedae Parameters for the Primary \label{tab:lambda_Andparams}}
\tablecolumns{5}
\tablewidth{0pt}
\tablehead{
\colhead{Observed Parameters} &
\colhead{Value} &
\colhead{Source} &
\colhead{Values from literature} & 
\colhead{Literature reference}
%\colhead{Values from \cite{parks:2021}}
}
\startdata
$R_{\star}$ (mas) & 1.371 \pm 0.005 & This work & 1.379 \pm 0.025 & \cite{parks:2021} \\ 
Limb-darkening coefficient & 0.231 \pm 0.024 & This work & 0.229 \pm 0.111 & \cite{parks:2021} \\ 
Inclination (deg) & 85.63 \pm 2.32 & This work & 70.35 \pm 6.7\tablenotemark{d} & \cite{parks:2021} \\ 
Position Angle (deg) & 26.09 \pm 0.82 & This work & 21.6 \pm 7.5\tablenotemark{d} & \cite{parks:2021} \\ 
Rotation Period (days) & 54.2 & This work & 56.9 \pm 8.8\tablenotemark{d} & \cite{parks:2021} \\
\hline
Physical parameters & & & \\
\hline
$R_{\star}$ ($R_{\odot}$) & 7.787 \pm 0.053 & This work\tablenotemark{a} & 7.831^{+0.067}_{-0.065} & \cite{parks:2021}\\ 
$T_{\mathrm{eff}}$ (K) & 4800 \pm 100 & \cite{drake:2011} & - & $-$ \\
log $g$ & 2.75\pm 0.25 & \cite{drake:2011} & - & $-$ \\
$M_{\star}$ ($M_{\odot}$) & 1.24 \pm 0.72 & This work\tablenotemark{b} & 1.3^{+1.0}_{-0.6} & \cite{drake:2011} \\
log $L/L_{\odot}$ & 1.46 \pm 0.04 & This work\tablenotemark{c} & 1.37 \pm 0.04 & \cite{drake:2011} \\
distance (pc) & 26.41 \pm 0.15 & \cite{vanleeuwen:2007} & - & $-$ \\
\enddata
\tablenotetext{a}{Based on the angular radius from this work and the distance from \cite{vanleeuwen:2007}.}
\tablenotetext{b}{Based on the physical radius from this work and the log $g$ from \cite{drake:2011}.}
\tablenotetext{c}{Based on the physical radius from this work and the effective temperature from \cite{drake:2011}.}
\tablenotetext{d}{Since \cite{parks:2021} had multiple values reported for the same parameter, we show the averages of the respective parameter here.}
\tablecomments{The observed parameters were optimized through a bootstrap approach with the exception of the rotation period, which was fixed. We take our fixed rotation period parameter directly from the best model in \texttt{SIMTOI}.}
\end{deluxetable*}


==> Martinez_etal_2021 - Dynamical Surface Imaging of lambda Andromedae/tables/observations.tex <==
\begin{deluxetable*}{ccccccl}[t!]
\tablenum{1}
\tablecaption{CHARA Array observations \label{tab:observe}}
\tablecolumns{7}
\tablewidth{0pt}
\tablehead{
\colhead{UT date} &
\colhead{Average} &
\colhead{Baselines} &
\colhead{Number of} &
\colhead{Number of} &
\colhead{Rotation Phase} &
\colhead{Calibrators} \vspace{-5pt} \\
\colhead{} &
\colhead{MJD} &
\colhead{} &
\colhead{$|V|^2$ points} &
\colhead{Closure Phases} &
\colhead{of Primary} &
\colhead{}
}
\startdata
2010 Aug 02 & 55410.4 & S1-E1-W1-W2 & 167 & 88 & 0.0 & 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 03 & 55411.3 & S1-E1-W1-W2 & 454 & 264 & 0.012 & $\sigma$ Cyg, 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 10 & 55418.3 & S1-E1-W1-W2 & 425 & 288 & 0.146 & $\sigma$ Cyg, 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 11 & 55419.3 & S1-E1-W1-W2 & 215 & 136 & 0.164 & $\sigma$ Cyg, 7 And, 37 And \\
2010 Aug 18 & 55426.3 & S1-E1-W1-W2 & 429 & 272 & 0.293 & $\sigma$ Cyg, 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 19 & 55427.3 & S1-E1-W1-W2 & 406 & 264 & 0.312 & $\sigma$ Cyg, 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 24 & 55432.3 & S1-E1-W1-W2 & 526 & 320 & 0.404 & $\sigma$ Cyg, 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Aug 25 & 55433.3 & S2-E2-W1-W2 & 120 & 72 & 0.423 & $\sigma$ Cyg, 7 And, 37 And \\
2010 Sep 02 & 55441.3 & S1-E1-W1-W2 & 522 & 336 & 0.570 & 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Sep 03 & 55442.3 & S1-E1-W1-W2 & 588 & 352 & 0.589 & 7 And, 37 And \\
 & & S2-E2-W1-W2 & & \\
2010 Sep 10 & 55449.3 & S2-E2-W1-W2 & 336 & 192 & 0.718 & 7 And, 37 And \\
2011 Sep 02 & 55806.5 & W1-S2-S1-E1-E2-W2 & 360 & 432 & 0.310 & $\sigma$ Cyg, 7 And, 22 And, HR 653 \\ 
2011 Sep 06 & 55810.5 & W1-S2-S1-E1-E2-W2 & 392 & 376 & 0.384 & $\sigma$ Cyg, 7 And, 22 And, HR 653 \\ 
2011 Sep 10 & 55814.5 & W1-S2-S1-E1-E2-W2 & 360 & 432 & 0.458 & 7 And, 22 And \\ 
2011 Sep 14 & 55818.5 & W1-S2-S1-E1-E2-W2 & 864 & 1104 & 0.532 & 7 And, 22 And, HR 653 \\ 
2011 Sep 19 & 55823.5 & W1-S2-S1-E1-E2-W2 & 808 & 1120 & 0.624 & 7 And, 22 And, HR 653 \\
2011 Sep 24 & 55828.5 & W1-S2-S1-E1-E2-W2 & 200 & 240 & 0.716 & 7 And, 22 And, HR 653, $\eta$ Aur \\
\enddata
\tablecomments{Here we list the UT date, the average modified Julian date of the night of observation, the baselines used in their corresponding configuration, the number of useful squared visibility points obtained for the night, the number of useful closure phase points obtained for the night, the rotation phase for the primary star in $\lambda$ And, and the calibrator stars that were used for each corresponding night. The rotation phase is derived by using the first observation in 2010 as the zero point.}
\end{deluxetable*}

==> Martinez_etal_2021 - Dynamical Surface Imaging of lambda Andromedae/tables/orbit_params.tex <==
\begin{deluxetable}{lCc}%[t!]
\tablenum{4}
\tablecaption{Orbital Parameters \& Secondary Parameters \label{tab:orbitparams}}
\tablecolumns{3}
\tablewidth{0pt}
\tablehead{
\colhead{Observable Parameters} &
\colhead{Value} &
\colhead{Source}
}
\startdata
$R_{\star}$ (mas) & 0.03 \pm ? & This work \\
separation (mas) & 6.12 \pm ? & This work \\ 
\hline
Physical parameters & & \\
\hline
$R_{\star}$ ($R_{\odot}$) & 0.19 \pm ? & This work\tablenotemark{a} \\
$M_{\star}$ ($M_{\odot}$) & 0.15^{0.09}_{0.05} & This work\tablenotemark{b} \\
log $L/L_{\odot}$ & 1.46 \pm 0.04 & This work\tablenotemark{c} \\
\tablenotetext{a}{Based on the angular radius from this work and the distance from \cite{vanleeuwen:2007}.}
\tablenotetext{b}{Based on the physical radius from this work and the log $g$ from \cite{drake:2011}.}
\tablenotetext{c}{Based on the physical radius from this work and the effective temperature from \cite{drake:2011}.}

\tablecomments{}
\end{deluxetable}


==> Martinez_etal_2021 - Dynamical Surface Imaging of lambda Andromedae/tables/simtoi_tab.tex <==
\begin{deluxetable*}{ccccc}%[t!]
\tablenum{3}
\tablecaption{\texttt{SIMTOI} Model Results \label{tab:simtoi_results}}
\tablecolumns{5}
\tablewidth{0pt}
\tablehead{
\colhead{Number of} &
\multicolumn{2}{c}{Importance Nested} &
\multicolumn{2}{c}{$\chi_{\nu}^2$} \vspace{-5pt} \\
\colhead{spots} &
\multicolumn{2}{c}{Sampling value (ln $Z$)} &
\multicolumn{2}{c}{} \\
\cline{2-5} \vspace{-15pt} \\
& \colhead{2010 data} & \colhead{2011 data} & \colhead{2010 data} & \colhead{2011 data} \vspace{-15pt} \\
}
\startdata
3 & -67599.448761 & 10433.734767 & 56.855263 & 8.020829 \\ 
4 &  -5968.401012 & 36157.820383 & 17.114268 & 3.102330 \\ 
5 &   1420.128960 & 32785.721919 & 11.372939 & 3.710609 \\
6 & -45295.096429 & 30193.016672 & 38.679240 & 4.211333 \\ 
\hline
Physical parameters & Value & & \\
(4 spot model based on 2011 data) & & & \\
\hline
\multicolumn{1}{l}{$R_{\star}$ (mas)} & 1.37 & & \\ 
\multicolumn{1}{l}{Limb-darkening coefficient} & 0.22 & & \\
\multicolumn{1}{l}{Inclination (deg)} & 86.4 & & \\
\multicolumn{1}{l}{Position Angle (deg)} & 26.7 & & \\
\multicolumn{1}{l}{Rotation Period (days)} & 54.2 & & \\ 
\enddata
\tablecomments{Higher ln $Z$ value is better, lower $\chi_{\nu}^2$ is better. No error bars are calculated since the models from \texttt{SIMTOI} using Multinest does not currently generate reliable error bars. We rely on the imaging results for more precise measurements and calculation of errors.}
\end{deluxetable*}

==> tables/orbit_params.tex <==
\begin{deluxetable}{lCc}%[t!]
\tablenum{4}
\tablecaption{Orbital Parameters \& Secondary Parameters \label{tab:orbitparams}}
\tablecolumns{3}
\tablewidth{0pt}
\tablehead{
\colhead{Observable Parameters} &
\colhead{Value} &
\colhead{Source}
}
\startdata
$R_{\star}$ (mas) & 0.03 \pm ? & This work \\
separation (mas) & 6.12 \pm ? & This work \\ 
\hline
Physical parameters & & \\
\hline
$R_{\star}$ ($R_{\odot}$) & 0.19 \pm ? & This work\tablenotemark{a} \\
$M_{\star}$ ($M_{\odot}$) & 0.15^{0.09}_{0.05} & This work\tablenotemark{b} \\
log $L/L_{\odot}$ & 1.46 \pm 0.04 & This work\tablenotemark{c} \\
\tablenotetext{a}{Based on the angular radius from this work and the distance from \cite{vanleeuwen:2007}.}
\tablenotetext{b}{Based on the physical radius from this work and the log $g$ from \cite{drake:2011}.}
\tablenotetext{c}{Based on the physical radius from this work and the effective temperature from \cite{drake:2011}.}

\tablecomments{}
\end{deluxetable}

